Raising Student Completion Rates with Adaptive Curriculum and Contextual Bandits

We present an adaptive learning Intelligent Tutoring System, which uses model-based reinforcement learning in the form of contextual bandits to assign learning activities to students. The model is trained on the trajectories of thousands of students in order to maximize their exercise completion rates and continues to learn online, automatically adjusting itself to new activities. A randomized controlled trial with students shows that our model leads to superior completion rates and significantly improved student engagement when compared to other approaches. Our approach is fully-automated unlocking new opportunities for learning experience personalization.

==> temp_sources.tex <==
linucb
https://arxiv.org/pdf/1003.0146.pdf

https://papers.nips.cc/paper/2007/file/4b04a686b0ad13dce35fa99fa4161c65-Paper.pdf


Copy:
@article{Li2010,
   title={A contextual-bandit approach to personalized news article recommendation},
   url={http://dx.doi.org/10.1145/1772690.1772758},
   DOI={10.1145/1772690.1772758},
   journal={Proceedings of the 19th international conference on World wide web - WWW  ’10},
   publisher={ACM Press},
   author={Li, Lihong and Chu, Wei and Langford, John and Schapire, Robert E.},
   year={2010},
   }
   
@article{Zhou2015,
  author    = {Li Zhou},
  title     = {A Survey on Contextual Multi-armed Bandits},
  journal   = {CoRR},
  volume    = {abs/1508.03326},
  year      = {2015},
  url       = {http://arxiv.org/abs/1508.03326},
  eprinttype = {arXiv},
  eprint    = {1508.03326},
  timestamp = {Sun, 06 Sep 2020 22:24:21 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/Zhou15c.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org},
}

@book{Sutton2018,
author = {Sutton, Richard S. and Barto, Andrew G.},
title = {Reinforcement Learning: An Introduction},
year = {2018},
isbn = {0262039249},
publisher = {A Bradford Book},
address = {Cambridge, MA, USA},
}

@article{Robbins1952,
author = {Herbert Robbins},
title = {{Some aspects of the sequential design of experiments}},
volume = {58},
journal = {Bulletin of the American Mathematical Society},
number = {5},
publisher = {American Mathematical Society},
pages = {527 -- 535},
year = {1952},
doi = {bams/1183517370},
URL = {https://doi.org/}
}

@article{Auer2002,
author = {Auer, Peter and Cesa-Bianchi, Nicolò and Fischer, Paul},
year = {2002},
month = {05},
pages = {235-256},
title = {Finite-time Analysis of the Multiarmed Bandit Problem},
volume = {47},
journal = {Machine Learning},
doi = {10.1023/A:1013689704352}
}

@article{Auer2003,
author = {Auer, Peter and Cesa-Bianchi, Nicol\`{o} and Freund, Yoav and Schapire, Robert E.},
title = {The Nonstochastic Multiarmed Bandit Problem},
year = {2003},
issue_date = {2003},
publisher = {Society for Industrial and Applied Mathematics},
address = {USA},
volume = {32},
number = {1},
issn = {0097-5397},
url = {https://doi.org/10.1137/S0097539701398375},
doi = {10.1137/S0097539701398375},
month = {jan},
pages = {48–77},
numpages = {30},
keywords = {unknown matrix games, adversarial bandit problem}
}

@inproceedings{Langford2007,
author = {Langford, John and Zhang, Tong},
year = {2007},
month = {01},
pages = {},
title = {The Epoch-Greedy Algorithm for Multi-armed Bandits with Side Information.}
}

@article{Auer2003_2,
author = {Auer, Peter},
title = {Using Confidence Bounds for Exploitation-Exploration Trade-Offs},
year = {2003},
issue_date = {3/1/2003},
publisher = {JMLR.org},
volume = {3},
number = {null},
issn = {1532-4435},
month = {mar},
pages = {397–422},
numpages = {26},
keywords = {bandit problem, reinforcement learning, online Learning, exploitation-exploration, linear value function}
}

@inproceedings{Chu2011,
  title={Contextual Bandits with Linear Payoff Functions},
  author={Wei Chu and Lihong Li and L. Reyzin and Robert E. Schapire},
  booktitle={AISTATS},
  year={2011}
}

@article{Singla2021,
  author    = {Adish Singla and
               Anna N. Rafferty and
               Goran Radanovic and
               Neil T. Heffernan},
  title     = {Reinforcement Learning for Education: Opportunities and Challenges},
  journal   = {CoRR},
  volume    = {abs/2107.08828},
  year      = {2021},
  url       = {https://arxiv.org/abs/2107.08828},
  eprinttype = {arXiv},
  eprint    = {2107.08828},
  timestamp = {Thu, 22 Jul 2021 11:14:11 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2107-08828.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Lopes2013,
  author    = {Manuel Lopes and
               Benjamin Clement and
               Didier Roy and
               Pierre{-}Yves Oudeyer},
  title     = {Multi-Armed Bandits for Intelligent Tutoring Systems},
  journal   = {CoRR},
  volume    = {abs/1310.3174},
  year      = {2013},
  url       = {http://arxiv.org/abs/1310.3174},
  eprinttype = {arXiv},
  eprint    = {1310.3174},
  timestamp = {Thu, 14 Oct 2021 09:18:21 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/LopesCRO13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Fahid2021,
  title={Adaptively Scaffolding Cognitive Engagement with Batch Constrained Deep Q-Networks},
  author={Fahid, Fahmid Morshed and Rowe, Jonathan P and Spain, Randall D and Goldberg, Benjamin S and Pokorny, Robert and Lester, James},
  booktitle={International Conference on Artificial Intelligence in Education},
  pages={113--124},
  year={2021},
  organization={Springer}
}

@article{Chi2011,
author = {Chi, Min and Vanlehn, Kurt and Litman, Diane and Jordan, Pamela},
year = {2011},
month = {04},
pages = {137-180},
title = {Empirically evaluating the application of reinforcement learning to the induction of effective and adaptive pedagogical strategies},
volume = {21},
journal = {User Model. User-Adapt. Interact.},
doi = {10.1007/s11257-010-9093-1}
}

@article{Doroudi2019,
author = {Doroudi, Shayan and Aleven, Vincent and Brunskill, Emma},
year = {2019},
month = {11},
pages = {},
title = {Where’s the Reward?: A Review of Reinforcement Learning for Instructional Sequencing},
volume = {29},
journal = {International Journal of Artificial Intelligence in Education},
doi = {10.1007/s40593-019-00187-x}
}

@inproceedings{Aleven2016,
  title={Instruction Based on Adaptive Learning Technologies},
  author={Vincent Aleven and Elizabeth A. McLaughlin and Amos Glenn and K. Koedinger},
  year={2016}
}

@inproceedings{Williams2016,
  author = {Williams, Joseph Jay and Kim, Juho and Rafferty, Anna and Maldonado, Samuel and Gajos, Krzysztof Z. and Lasecki, Walter S. and Heffernan, Neil},
  title = {AXIS: Generating Explanations at Scale with Learnersourcing and Machine Learning},
  booktitle = {Proceedings of the Third (2016) ACM Conference on Learning @ Scale},
  series = {L@S '16},
  year = {2016},
  isbn = {978-1-4503-3726-7},
  location = {Edinburgh, Scotland, UK},
  pages = {379--388},
  numpages = {10},
    doi = {10.1145/2876034.2876042},
  acmid = {2876042},
  publisher = {ACM},
  address = {New York, NY, USA},
  keywords = {adaptive learning, crowdsourcing, explanation, learnersourcing, learning at scale, machine learning},
        award = {Honorable Mention},
}

@inproceedings{Patikorn2020,
author = {Patikorn, Thanaporn and Heffernan, Neil T.},
title = {Effectiveness of Crowd-Sourcing On-Demand Assistance from Teachers in Online Learning Platforms},
year = {2020},
isbn = {9781450379519},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3386527.3405912},
doi = {10.1145/3386527.3405912},
pages = {115–124},
numpages = {10},
keywords = {tutored problem solving, assistments, learning management system, crowd-sourcing},
location = {Virtual Event, USA},
series = {L@S '20}
}

@inbook{Erickson2020,
author = {Erickson, John A. and Botelho, Anthony F. and McAteer, Steven and Varatharaj, Ashvini and Heffernan, Neil T.},
title = {The Automated Grading of Student Open Responses in Mathematics},
year = {2020},
isbn = {9781450377126},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3375462.3375523},
booktitle = {Proceedings of the Tenth International Conference on Learning Analytics &amp; Knowledge},
pages = {615–624},
numpages = {10}
}

@article{Whitehill2017,
author = {Whitehill, Jacob and Movellan, Javier},
year = {2017},
month = {04},
pages = {1-1},
title = {Approximately Optimal Teaching of Approximately Optimal Learners},
volume = {PP},
journal = {IEEE Transactions on Learning Technologies},
doi = {10.1109/TLT.2017.2692761}
}

@inproceedings{Liu2014,
  title={Trading Off Scientific Knowledge and User Learning with Multi-Armed Bandits},
  author={Yun-En Liu and Travis Mandel and Emma Brunskill and Zoran Popovic},
  booktitle={EDM},
  year={2014}
}

@inbook{Williams2018,
author = {Williams, Joseph Jay and Rafferty, Anna N. and Tingley, Dustin and Ang, Andrew and Lasecki, Walter S. and Kim, Juho},
title = {Enhancing Online Problems Through Instructor-Centered Tools for Randomized Experiments},
year = {2018},
isbn = {9781450356206},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3173574.3173781},
booktitle = {Proceedings of the 2018 CHI Conference on Human Factors in Computing Systems},
pages = {1–12},
numpages = {12}
}

@article{anderson1985,
  title={{Intelligent tutoring systems}},
  author={Anderson, John R and Boyle, C Franklin and Reiser, Brian J},
  journal={Science},
  volume={228},
  number={4698},
  pages={456--462},
  year={1985},
  publisher={American Association for the Advancement of Science}
}

@article{nye2014,
  title={{AutoTutor and family: A review of 17 years of natural language tutoring}},
  author={Nye, Benjamin D and Graesser, Arthur C and Hu, Xiangen},
  journal={International Journal of Artificial Intelligence in Education},
  volume={24},
  number={4},
  pages={427--469},
  year={2014},
  publisher={Springer}
}

@article{Arroyo,
author = {Arroyo, Ivon and Beal, Carole and Bergman, Ari and Lindenmuth, Mike and Marshall, David and Woolf, Beverly},
year = {2003},
title = {Intelligent Tutoring for high-stakes achievement tests},
journal = {Eleventh International Conference on Artificial Intelligence and Education},
}

@inproceedings{albacete2019impact,
  title={{The Impact of Student Model Updates on Contingent Scaffolding in a Natural-Language Tutoring System}},
  author={Albacete, Patricia and Jordan, Pamela and Katz, Sandra and Chounta, Irene-Angelica and McLaren, Bruce M},
  booktitle={International Conference on Artificial Intelligence in Education},
  pages={37--47},
  year={2019},
  organization={Springer}
}

@inproceedings{chi2011instructional,
author = {Chi, Min and Koedinger, Kenneth and Gordon, Geoffrey and Jordan, Pamela and Vanlehn, Kurt},
year = {2011},
month = {01},
pages = {61-70},
title = {{Instructional Factors Analysis: A Cognitive Model For Multiple Instructional Interventions}},
booktitle = {EDM 2011 - Proceedings of the 4th International Conference on Educational Data Mining}
}

@article{Lin,
title = {{Data mining for providing a personalized learning path in creativity: An application of decision trees}},
journal = "Computers \& Education",
volume = "68",
pages = "199 - 210",
year = "2013",
issn = "0360-1315",
doi = "https://doi.org/10.1016/j.compedu.2013.05.009",
url = "http://www.sciencedirect.com/science/article/pii/S0360131513001309",
author = "Chun Fu Lin and Yu-chu Yeh and Yu Hsin Hung and Ray I Chang",
keywords = "Intelligent tutoring systems, Architectures for educational technology systems, Teaching/learning strategies",
abstract = "Customizing a learning environment to optimize personal learning has recently become a popular trend in e-learning. Because creativity has become an essential skill in the current e-learning epoch, this study aims to develop a personalized creativity learning system (PCLS) that is based on the data mining technique of decision trees to provide personalized learning paths for optimizing the performance of creativity. The PCLS includes a series of creativity tasks as well as a questionnaire regarding several key variables. Ninety-two college students were included in this study to examine the effectiveness of the PCLS. The experimental results show that, when the learning path suggested by a hybrid decision tree is employed, the learners have a 90\% probability of obtaining an above-average creativity score, which suggests that the employed data mining technique can be a good vehicle for providing adaptive learning that is related to creativity. Moreover, the findings in this study shed light on what components should be accounted for when designing a personalized creativity learning system as well as how to integrate personalized learning and game-based learning into a creative learning program to maximize learner motivation and learning effects."
}

@inproceedings{munshi2019personalization,
  title={Personalization in OELEs: Developing a Data-Driven Framework to Model and Scaffold SRL Processes},
  author={Munshi, Anabil and Biswas, Gautam},
  booktitle={International Conference on Artificial Intelligence in Education},
  pages={354--358},
  year={2019},
  organization={Springer}
}

@inproceedings{rus2014macro,
  title={Macro-adaptation in conversational intelligent tutoring matters},
  author={Rus, Vasile and Stefanescu, Dan and Baggett, William and Niraula, Nobal and Franceschetti, Don and Graesser, Arthur C},
  booktitle={International Conference on Intelligent Tutoring Systems},
  pages={242--247},
  year={2014},
  organization={Springer}
}

@inproceedings{rus2014deeptutor,
  title={DeepTutor: towards macro-and micro-adaptive conversational intelligent tutoring at scale},
  author={Rus, Vasile and Stefanescu, Dan and Niraula, Nobal and Graesser, Arthur C},
  booktitle={Proceedings of the first ACM conference on Learning@ scale conference},
  pages={209--210},
  year={2014}
}

@article{anderson1985intelligent,
  title={Intelligent tutoring systems},
  author={Anderson, John R and Boyle, C Franklin and Reiser, Brian J},
  journal={Science},
  volume={228},
  number={4698},
  pages={456--462},
  year={1985},
  publisher={American Association for the Advancement of Science}
}

@article{nye2014autotutor,
  title={AutoTutor and family: A review of 17 years of natural language tutoring},
  author={Nye, Benjamin D and Graesser, Arthur C and Hu, Xiangen},
  journal={International Journal of Artificial Intelligence in Education},
  volume={24},
  number={4},
  pages={427--469},
  year={2014},
  publisher={Springer}
}

@article{anania1983influence,
  title={The Influence of Instructional Conditions on Student Learning and Achievement.},
  author={Anania, Joanne},
  journal={Evaluation in Education: An International Review Series},
  volume={7},
  number={1},
  pages={3--76},
  year={1983},
  publisher={ERIC}
}

@article{bloom19842,
  title={The 2 sigma problem: The search for methods of group instruction as effective as one-to-one tutoring},
  author={Bloom, Benjamin S},
  journal={Educational researcher},
  volume={13},
  number={6},
  pages={4--16},
  year={1984},
  publisher={Sage Publications Sage CA: Thousand Oaks, CA}
}

@phdthesis{burke1983students,
  title={Students' potential for learning contrasted under tutorial and group approaches to instruction},
  author={Burke, Arthur Joseph},
  year={1983},
  school={University of Chicago, Joseph Regenstein Library, Department of Photoduplication}
}

@article{Hrastinski,
author = {Stefan Hrastinski and Stefan Stenbom and Simon Benjaminsson and Malin Jansson},
title = {Identifying and exploring the effects of different types of tutor questions in individual online synchronous tutoring in mathematics},
journal = {Interactive Learning Environments},
volume = {0},
number = {0},
pages = {1--13},
year  = {2019},
publisher = {Routledge},
doi = {10.1080/10494820.2019.1583674},
URL = {https://doi.org/10.1080/10494820.2019.1583674},
eprint = {https://doi.org/10.1080/10494820.2019.1583674}
}

@book{Wenger,
author = {Wenger, \'{E}tienne},
year = {1987},
publisher = {Los Altos, CA: Morgan Kaufmann},
title = {{Artificial Intelligence and Tutoring Systems}}
}

@article{Hone,
author = {Hone, Kate and El Said, Ghada},
year = {2016},
month = {03},
pages = {157--168},
title = {{Exploring the factors affecting MOOC retention: A survey study}},
volume = {98},
journal = {Computers \& Education},
doi = {10.1016/j.compedu.2016.03.016}
}

@article{kulik2016effectiveness,
  title={{Effectiveness of intelligent tutoring systems: a meta-analytic review}},
  author={Kulik, James A and Fletcher, JD},
  journal={Review of educational research},
  volume={86},
  number={1},
  pages={42--78},
  year={2016},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@article{VanLehn,
author = {Kurt VanLehn},
title = {{The Relative Effectiveness of Human Tutoring, Intelligent Tutoring Systems, and Other Tutoring Systems}},
journal = {Educational Psychologist},
volume = {46},
number = {4},
pages = {197-221},
year  = {2011},
publisher = {Routledge},
doi = {10.1080/00461520.2011.611369},
URL = { 
        https://doi.org/10.1080/00461520.2011.611369
},
eprint = { 
        https://doi.org/10.1080/00461520.2011.611369
    
}
}


@article{Graesser,
title = "Assessment with computer agents that engage in conversational dialogues and trialogues with learners",
journal = "Computers in Human Behavior",
volume = "76",
pages = "607 - 616",
year = "2017",
issn = "0747-5632",
doi = "https://doi.org/10.1016/j.chb.2017.03.041",
url = "http://www.sciencedirect.com/science/article/pii/S074756321730198X",
author = "Arthur C. Graesser and Zhiqiang Cai and Brent Morgan and Lijia Wang",
keywords = "Conversational agents, Conversation-based assessment, Intelligent tutoring systems, Trialogues",
abstract = "This article describes conversation-based assessments with computer agents that interact with humans through chat, talking heads, or embodied animated avatars. Some of these agents perform actions, interact with multimedia, hold conversations with humans in natural language, and adaptively respond to a person’s actions, verbal contributions, and emotions. Data are logged throughout the interactions in order to assess the individual’s mastery of subject matters, skills, and proficiencies on both cognitive and noncognitive characteristics. There are different agent-based designs that focus on learning and assessment. Dialogues occur between one agent and one human, as in the case of intelligent tutoring systems. Three-party conversations, called trialogues, involve two agents interacting with a human. The two agents can take on different roles (such as tutors and peers), model actions and social interactions, stage arguments, solicit help from the human, and collaboratively solve problems. Examples of assessment with these agent-based environments are presented in the context of intelligent tutoring, educational games, and interventions to help struggling adult readers. Most of these involve assessment at varying grain sizes to guide the intelligent interaction, but conversation-based assessment with agents is also currently being used in high stakes assessments."
}


@InProceedings{Wu,
author={Wu, Longkai
and Looi, Chee-Kit},
editor={Aleven, Vincent
and Kay, Judy
and Mostow, Jack},
title={{Agent Prompts: Scaffolding Students for Productive Reflection in an Intelligent Learning Environment}},
booktitle="Intelligent Tutoring Systems",
year={2010},
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="426--428",
abstract="Recent research has emphasized the importance of reflection for students in an intelligent learning environment. This study tries to investigate whether agent prompts, acting as scaffolding, can promote students' reflection when they act as tutor through teaching the agent tutee in a learning-by-teaching environment. Two types of agent prompts are contrasted in this research, both from the perspective of a tutee, differing in their specificity. Reflective prompts are content-independent tutee questions, aiming at fostering students' general reflection on metacognitive strategies and beliefs. Interactive prompts, on the other hand, are content-dependent tutee questions that encourage students' specific reflection on domain-related and task-specific skills and articulation of their explanatory responses. The result indicates that designers on intelligent learning environment should concentrate on fostering students to reflect on their metacognitive strategies and beliefs, and allow students to take responsibility for directing their own learning autonomy.",
isbn="978-3-642-13437-1"
}

@inproceedings{piano2018,
  title={{Automatic Curriculum Generation Applied to Teaching Novices a Short Bach Piano Segment}},
  author={Brunskill, Emma and Mu, Tong and Goel, Karan and Bragg, Jonathan},
  year={2018}, 
  booktitle={NeurIPS Demonstrations}
}

@inproceedings{mu2018combining,
  title={Combining adaptivity with progression ordering for intelligent tutoring systems},
  author={Mu, Tong and Wang, Shuhan and Andersen, Erik and Brunskill, Emma},
  booktitle={Proceedings of the fifth annual ACM conference on learning at scale},
  pages={1--4},
  year={2018}
}

@article{clement2013multi,
  title={Multi-armed bandits for intelligent tutoring systems},
  author={Clement, Benjamin and Roy, Didier and Oudeyer, Pierre-Yves and Lopes, Manuel},
  journal={arXiv preprint arXiv:1310.3174},
  year={2013}
}

@inproceedings{Mui2021,
  title={Multi-armed Bandit Algorithms for Adaptive Learning: A Survey},
  author={Mui, John and Lin, Fuhua and Dewan, M.},
  booktitle={International Conference on Artificial Intelligence in Education},
  pages={273--278},
  year={2021},
  organization={Springer}
}

@article{Segal2018,
  author    = {Avi Segal and
               Yossi Ben David and
               Joseph Jay Williams and
               Kobi Gal and
               Yaar Shalom},
  title     = {Combining Difficulty Ranking with Multi-Armed Bandits to Sequence
               Educational Content},
  journal   = {CoRR},
  volume    = {abs/1804.05212},
  year      = {2018},
  url       = {http://arxiv.org/abs/1804.05212},
  eprinttype = {arXiv},
  eprint    = {1804.05212},
  timestamp = {Mon, 13 Aug 2018 16:46:34 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1804-05212.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Lan2016,
  title={A Contextual Bandits Framework for Personalized Learning Action Selection.},
  author={Lan, Andrew S and Baraniuk, Richard G},
  booktitle={EDM},
  pages={424--429},
  year={2016}
}

@article{Sutton1991,
author = {Sutton, Richard S.},
title = {Dyna, an Integrated Architecture for Learning, Planning, and Reacting},
year = {1991},
issue_date = {Aug. 1991},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {2},
number = {4},
issn = {0163-5719},
url = {https://doi.org/10.1145/122344.122377},
doi = {10.1145/122344.122377},
journal = {SIGART Bull.},
month = {jul},
pages = {160–163},
numpages = {4}
}

@article{Brafman2003,
author = {Brafman, Ronen I. and Tennenholtz, Moshe},
title = {R-Max - a General Polynomial Time Algorithm for near-Optimal Reinforcement Learning},
year = {2003},
issue_date = {3/1/2003},
publisher = {JMLR.org},
volume = {3},
number = {null},
issn = {1532-4435},
url = {https://doi.org/10.1162/153244303765208377},
doi = {10.1162/153244303765208377},
journal = {J. Mach. Learn. Res.},
month = {mar},
pages = {213–231},
numpages = {19},
keywords = {reinforcement learning, learning in games, stochastic games, Markov decision processes, provably efficient learning}
}
